Absurd World: A Simple Yet Powerful Method to Absurdify the Real-world for Probing LLM Reasoning Capabilities

While extremely powerful and versatile at various tasks, the thinking capabilities of large language models (LLMs) are often put under scrutiny as they sometimes fail to solve problems that humans can systematically solve. However, recent literature focuses on breaking LLM reasoning with increasingly complex problems, and whether an LLM is robust in simple logical reasoning remains underexplored. This paper proposes Absurd World, a benchmarking framework, to test LLMs against altered realism, where scenarios are logically coherent, and humans can easily solve the tasks. Absurd World breaks a real-world model into symbols, actions, sequences, and events, which are automatically altered to create absurd worlds where the logic to solve the tasks remains the same. It evaluates a large collection of models with simple and advanced prompting techniques, and proves that it is an effective tool to determine LLMs' ability to think logically, ignoring the patterns learned from the real world. One can use this framework to extensively test an LLM against a real-world problem to verify whether the LLM's reasoning capability is robust against variations of the task.

==> tables/initial_result.tex <==
\begin{table}[h]
\centering
\caption{Performance of different rulesets for the inital Determine Outcome task. Reported numbers are average scores (higher is better).}
\label{tab:ruleset_results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\textbf{Model Category} & \textbf{REAL} & \textbf{MISSING} & \textbf{LEAST} & \textbf{ICE CREAM} & \textbf{CAR} & \textbf{SWITCH} & \textbf{MISS \& SWITCH} \\
\midrule
Cheap & 0.938 & 0.862 & 0.954 & 0.934 & 0.938 & 0.928 & 0.856 \\ 
Expensive & 0.849 & 0.720 & 0.810 & 0.853 & 0.841 & 0.844 & 0.721 \\
Reasoning & 0.985 & 0.988 & 0.995 & 0.990 & 0.995 & 0.993 & 0.990\\ 
\bottomrule
\end{tabular}
}
\end{table}


==> tables/models.tex <==
\begin{table}[ht]
\centering
\caption{Models categorized by cost and reasoning specialization.}
\label{tab:model_groups_vertical}
\begin{tabular}{l l}
\toprule
\textbf{Category} & \textbf{Model} \\
\midrule
\multirow{5}{*}{Cheap} 
    & google/gemini-2.0-flash-001 \\
    & openai/gpt-4o-mini \\
    & meta-llama/llama-4-maverick-17b-128e-instruct \\
    & qwen/qwen-2.5-72b-instruct \\
    & google/gemini-2.5-flash \\
\midrule
\multirow{7}{*}{Expensive} 
    & anthropic/claude-3-5-haiku \\
    & nousresearch/hermes-3-llama-3.1-405b \\
    & sao10k/l3.1-euryale-70b \\
    & meta-llama/llama-3.1-405b-instruct \\
    & thedrummer/skyfall-36b-v2 \\
    & openai/gpt-4.1-mini \\
    & google/gemma-2-27b-it \\
\midrule
\multirow{2}{*}{Reasoning} 
    & deepseek/deepseek-r1-0528 \\
    & nvidia/llama-3.1-nemotron-ultra-253b-v1 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/new_result.tex <==
\begin{table}[h]
\centering
\caption{Performance of different rulesets for Determine Outcome task. Reported numbers are average scores (higher is better).}
\label{tab:ruleset_results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\textbf{Model Category} & \textbf{REAL} & \textbf{MISSING} & \textbf{LEAST} & \textbf{ICE CREAM} & \textbf{CAR} & \textbf{SWITCH} & \textbf{MISS \& SWITCH} \\
\midrule
Cheap & $0.988$ & $0.956$ & $0.992$ & $0.988$ & $0.990$ & $0.984$ & $0.964$ \\
Expensive & $0.937$ & $0.846$ & $0.910$ & $0.950$ & $0.934$ & $0.933$ & $0.831$ \\
Reasoning & $1.000$ & $1.000$ & $1.000$ & $1.000$ & $1.000$ & $1.000$ & $1.000$ \\
\bottomrule
\end{tabular}}
\end{table}

==> tables/new_result_1.tex <==
\begin{table}[h]
\centering
\caption{Performance of different rulesets for Determine Outcome Few-Shot task. Reported numbers are average scores (higher is better).}
\label{tab:ruleset_results}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\textbf{Model Category} & \textbf{REAL} & \textbf{MISSING} & \textbf{LEAST} & \textbf{ICE CREAM} & \textbf{CAR} & \textbf{SWITCH} & \textbf{MISS \& SWITCH} \\
\midrule
Cheap & 0.918 & 0.906 & 0.914 & 0.914 & 0.92 & 0.898 & 0.886 \\
Expensive & 0.753 & 0.649 & 0.736 & 0.764 & 0.749 & 0.753 & 0.619 \\
Reasoning & 0.990 & 0.910 & 0.945 & 0.950 & 0.975 & 0.930 & 0.920 \\
\bottomrule
\end{tabular}
}
\end{table}


==> tables/rules-1.tex <==
\begin{table}[h]
\centering
\caption{Ruleset variations used in Absurd Soccer experiments. Each ruleset modifies the \textbf{REAL} ruleset in specific ways.}
\label{tab:rulesets-1}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lp{7.5cm}l@{}}
\toprule
\textbf{Ruleset} & \textbf{Modification} & \textbf{Change Type} \\
\midrule
REAL & No modification & N/A \\
\midrule
MISSING & Score increases by 1 when a shot \textit{misses} the net & Score mechanics \\
\midrule
LEAST & Team with the \textit{lowest} score wins & Score mechanics \\
\midrule
ICE CREAM & Teams earn ice cream instead of points when hitting the net & Score mechanics \\
\midrule
CAR & Teams earn cars instead of points when hitting the net & Score mechanics \\
\midrule
SWITCH & Teams shoot a \textit{net into a ball} (roles reversed) & Roles of symbols \\
\midrule
MISS \& SWITCH & Combination of MISSING and SWITCH & Both \\
\bottomrule
\end{tabular*}
\end{table}

==> tables/rules.tex <==
\begin{table}[h]
\centering
\caption{Variants of the game rules considered in our experiments. All are modifications of the \textit{REAL} ruleset.}
\label{tab:rulesets}
\begin{tabular}{l p{0.65\linewidth}}
\toprule
\textbf{Ruleset} & \textbf{Modification} \\
\midrule
REAL & No modification. \\
MISSING & Score increases by 1 when a shot misses. \\
LEAST & The team with the lowest score wins. \\
ICE CREAM & Team earns ice cream when hitting the net. \\
CAR & Team earns cars when hitting the net. \\
SWITCH & Teams shoot a net into a ball (roles reversed). \\
MISS \& SWITCH & Combination of \textsc{MISSING} and \textsc{SWITCH}. \\
\bottomrule
\end{tabular}
\end{table}

